Reflection on Code Contributor Demographics and Collaboration Patterns in the Rust Community

Open-source software communities thrive on global collaboration and contributions from diverse participants. This study explores the Rust programming language ecosystem to understand its contributors' demographic composition and interaction patterns. Our objective is to investigate the phenomenon of participation inequality in key Rust projects and the presence of diversity among them. We studied GitHub pull request data from the year leading up to the release of the latest completed Rust community annual survey in 2023. Specifically, we extracted information from three leading repositories: Rust, Rust Analyzer, and Cargo, and used social network graphs to visualize the interactions and identify central contributors and sub-communities. Social network analysis has shown concerning disparities in gender and geographic representation among contributors who play pivotal roles in collaboration networks and the presence of varying diversity levels in the sub-communities formed. These results suggest that while the Rust community is globally active, the contributor base does not fully reflect the diversity of the wider user community. We conclude that there is a need for more inclusive practices to encourage broader participation and ensure that the contributor base aligns more closely with the diverse global community that utilizes Rust.

==> sections/introduction.tex <==
\section{Introduction}
\label{intro}
Open-source software (OSS) communities form the backbone of contemporary software development, enabling collaboration among individuals worldwide who share a passion for technology and innovation. Participants often contribute in their free time and at a level that aligns with their expertise and availability, fostering an environment of collective growth and learning~\cite{lakhani2005hackers,motivation-in-oss}. Participants can contribute in various ways, such as reporting issues, submitting pull requests, conducting code reviews, and updating documentation. %These communities often operate under a Code of Conduct and exhibit complex organizational structures involving maintainers, core contributors, external contributors, and other roles essential for project sustainability.

The Rust programming language community offers a distinctive perspective on global engagement with emerging technologies. Despite Rust's reputation for being a highly admired language—ranked as the most admired programming language for eight consecutive years in the Stack Overflow 2024 survey~\footnote{\url{https://survey.stackoverflow.co/2024/}}—it addresses challenges inherent in low-level programming languages traditionally perceived as less accessible due to complexity. It also has impressive baked-in features such as memory safety, which led to massive growth and industry adoption over the past few years as an alternative to C/C++~\cite{common-bug-fix-pattterns-rust}. %Historically, communities like Linux have been viewed as less welcoming, often exhibiting gatekeeping behaviors\cite{incivility-linux-kernel} that can deter novice contributors.

In OSS projects hosted on platforms like GitHub, pull requests (PRs) are the primary mechanism for collaboration and communication. This process involves two pivotal roles:

\begin{itemize} 
\item \textbf{Author}: A user who submits a PR to propose merging their code changes into the repository. 
\item \textbf{Reviewer}: A user who examines PRs and approves or requests changes before merging them into the codebase. 
\end{itemize}

The interaction between authors and reviewers might encapsulate OSS communities' power dynamics and collaborative ethos. Understanding these relationships is crucial for analyzing the inclusivity and efficacy of the development process. On top of these roles, membership within the Rust GitHub organization is categorized into two primary levels: contributors and full members. Contributors are regular participants who have demonstrated consistent and independent contributions to the Rust compiler and related projects.\footnote{https://forge.rust-lang.org/compiler/membership.html} They are granted review (\texttt{r+}) privileges, access to specific bots, and the ability to modify labels and issues, enabling them to participate in the project's development and maintenance actively. Full members are seasoned contributors who continue their active participation and take on leadership roles, such as voting on Requests for Comments (RFCs) and shaping the project's strategic direction. The pathway to full membership involves consensus from existing team members and a demonstrated commitment to guiding the project's evolution. Additionally, the organization offers an alumni status for members who wish to take a temporary break from active contributions while retaining their affiliation. This structured membership framework ensures that the Rust community remains dynamic and inclusive, fostering an environment where contributors can grow and take on increasing responsibilities based on their dedication and impact.

This study aims to explore the human elements behind code contributions within the Rust community, particularly following the release of the Rust Annual Survey 2023. By analyzing PR data from the subsequent year, we seek to understand the diversity and collaborative dynamics among contributors. Specifically, we address the following refined research questions designed to capture the essence of our investigation:

\begin{enumerate} 
\item \textbf{How accurately does the diversity of active contributors reflect the broader Rust community's demographic composition?} \item \textbf{What are the collaboration patterns and interaction dynamics among Rust contributors?} \item \textbf{To what extent do sub-communities or contributor groups within the Rust ecosystem exhibit diversity?} 
\end{enumerate}

This study employs a comprehensive methodology to investigate the diversity and collaboration dynamics within the Rust programming community. We began by collecting pull request (PR) data from the top three Rust repositories—Rust, Rust Analyzer, and Cargo—over a one-year period preceding the Rust Annual Survey 2023. Utilizing the GitHub API, we extracted the usernames of PR authors and reviewers, enriching this dataset with demographic information such as geographic location and likely gender. We then constructed social network graphs in R, applying the Louvain community detection algorithm to identify sub-communities within the network. Diversity within these sub-communities was quantitatively assessed using Blau's Index. At the same time, various network metrics were calculated to evaluate the structure and dynamics of contributor interactions.

Our analysis revealed that the diversity of active contributors does not fully reflect the broader Rust community's demographic composition. Contributions are predominantly concentrated in a few countries, notably the United States and Germany, and exhibit a significant gender imbalance, with most contributors being male. Additionally, non-member contributors play a crucial role in the collaboration networks, often forming distinct clusters independent of official Rust organization members. Sub-communities demonstrate substantial geographic diversity; however, gender diversity remains notably low across all groups. 

The paper is organized as follows: Section \ref{related-work} reviews related work, Section \ref{methodology} explains the study's methods, and Section \ref{results} presents findings on contributor demographics and network structures. Section \ref{discussion} addresses the implications and suggests future research, while Section \ref{limitations-future-work} notes study limitations and future directions. Finally, Section \ref{conclusion} summarizes our contributions.
